Evolutionary Strategies with Analogy Partitions in p-guessing Games

In Keynesian Beauty Contests notably modeled by p-guessing games, players try to guess the average of guesses multiplied by p. Convergence of plays to Nash equilibrium has often been justified by agents' learning. However, interrogations remain on the origin of reasoning types and equilibrium behavior when learning takes place in unstable environments. When successive values of p can take values above and below 1, bounded rational agents may learn about their environment through simplified representations of the game, reasoning with analogies and constructing expectations about the behavior of other players. We introduce an evolutionary process of learning to investigate the dynamics of learning and the resulting optimal strategies in unstable p-guessing games environments with analogy partitions. As a validation of the approach, we first show that our genetic algorithm behaves consistently with previous results in persistent environments, converging to the Nash equilibrium. We characterize strategic behavior in mixed regimes with unstable values of p. Varying the number of iterations given to the genetic algorithm to learn about the game replicates the behavior of agents with different levels of reasoning of the level k approach. This evolutionary process hence proposes a learning foundation for endogenizing existence and transitions between levels of reasoning in cognitive hierarchy models.

==> archiv.tex <==

% ------------------------------------ %

% \clearpage

% \subsection*{Abstract}
% peut etre pouvez vous aussi reflechir a l'effet d'avoir différents p guessing game (on doit etre proche de p x la moyenne des annonces) et regarder l'effet de regrouper ces jeux dans une meme classe d'analogie.\\

% Mon intuition est que si tous les p sont inferieurs a 1, on devrait ne pouvoir soutenir que l'equilibre classique. 
% Par symetrie (généralement pas regarde) si tous les p sont plus grands que 1, on devrait seulement avoir la plus grande annonce (il faut peut etre imposer  que les annonces sont dans (1, 100) car si on inclut 0, il y aurait aussi 0 comme equilibre).

% le cas mixte avec certains p plus grands et d'autres plus petits que 1 est plus riche...\\

% j'ai conscience que votre idee est differente mais j'ai l'impression que quelque soit la manière d'aggreger le passe (toutes les périodes précédentes ou la derniere, on va converger vers l'eq de Nash, ce qui en fait decoule d'un resultat plus general sur les jeux dominance solvable comme le guessing game). La question en suspens est la vitesse de convergence. Intuitivement, plus la fenetre est courte (derniere periode seulement) plus on converge vite. Cette discussion me parait juste mais j'aimerais que vous la complétiez par ce que j'ai suggere plus haut (différents p guessing games). \\

% Si je résume en tenant compte de ces éléments, je pourrais proposer un modèle évolutionnaire pour comprendre comment évoluent les stratégies d'agents rassemblant en une classe d'analogies des p-guessing games aussi bien en dessous et au dessus de 1. Peut être établir deux benchmarks avec un environnement seulement avec p<1, un deuxième avec seulement p>1, et la démarche de comprendre ce qui se passe dans un cas mixte.\\

% Depuis nos premières discussions, j'ai beaucoup appris en dynamiques évolutionnaires, et conjointement j'ai appris à créer des algorithmes évolutionnaires, que j'utilise actuellement avec O. Compte. Avec ces outils, je pourrais tester la convergence vers la plus petite (respectivement plus grande) annonce quand une classe de jeux sont à p<1 (resp. p>1), et étudier cette convergence dans le cas mixte.\\

% Evolution of theories of mind \url{https://www.sciencedirect.com/science/article/pii/S0899825611002004}\\

% The use of certain heuristics or strategies in games is often interpreted as the outcome of a learning process in a stable enough environment. 
% While the so called $p$-guessing games have been intensively studied from theoretical and experimental perspectives, the neglected question of endogenous evolution of heuristics used by players in this setting may play an important role in explaining the convergence to Nash equilibrium achieved in experiments, unexplained with a level $k$ model with fixed types. This piece suggests an evolutionary foundation for the use of analogy-based reasoning \textcolor{blue}{(Jehiel, 1995)} in the context of these Keynesian Beauty Contests. Using $p$-guessing game performance in a replicator dynamics law of motion, this endogenous evolution of heuristics explains the adaptation of strategies in absence of perfect rationality and information. These model outlines the relevance of analogy-based reasoning as a successful and realistic heuristic, requiring lighter assumptions on agents' cognition than the standard pure rationality approach of $p$-guessing games.\\

% \textbf{Keywords}: Analogy-based reasoning, Beauty Contests, Bounded rationality, Evolutionary game theory

% \clearpage




% ------------------------------------------------------------ %
% \section{$p$-guessing Games}


% $N$ agents with individual types $\theta_i$ take part in this $p$-guessing game, where $p < 1$. Typically, this setting has been investigated for example with $p = \frac{1}{2}$ or $p = \frac{2}{3}$, namely that agents aim at guessing the half (or two thirds) of the average of the guesses done by the population of agents. For $p < 1$, an intuitive Nash equilibrium in infinite population games deals with guessing $0$. The optimal strategies for each level $k$ of rationality are:

% For an individual of level $k=1$, the action-guess $x_i^1$ is equal to the fraction $p$ of the expectation of the average guess of a population of level $0$ players.

% \begin{equation}
%     x_i^1 = p \mathbb{E}(x^0)
% \end{equation}

% For players of higher levels of reasoning, 

% \begin{equation}
%     x_i^k = p^k \mathbb{E}(x^{k-1})
% \end{equation}

% In this action form, the Nash equilibrium corresponds to the guess of an agent with infinite level of reasoning. Indeed, for $p < 1$, $\lim_{k \xrightarrow{} \infty} x_i^k = 0$.


% However, as the population size departs from this assumption to be finite or even small, guessing $0$ ...

% WHAT happens in experiments (add curve)

% why the standard model cannot explain this convergence...
% so how can we explain that? model to replicate this trend with realistic cognitive assumptions on agents

% \section{Analogy-based strategies in $p$-guessing Games}

% While a substantial part of the literature has devoted .... + REF
% Some important questions are left unsolved. Notably on the provenance of individual types, how one may transition between them, and the requirement of high degree of reasoning to obtain the experimental grounded convergence to the Nash equilibrium. Dealing with bounded rational actual economic agents, this requirement seems unlikely to be satisfied, and the convergence towards Nash equilibrium that most experiments observe may be judiciously explained by alternative mechanisms than arbitrary agents gain in rationality throughout the experiment.

% An alternative strategy encompasses a much relevant approach of learning with ... : analogy based reasoning. 

% Instead of using as argument of the best response function conditional on the type, the \textit{assumed} average guess of other players needs not to be assumed to correspond to the action of less-sophisticated-than-self individuals. This average guess of other players object is rather built over time through observation, by so doing converging to the actual average guess of the population. These analogy-reasoning agents may start with such erroneous priors, and may not be correct about their expectation of the behavior of other agents from the start. Nevertheless, this learning by analogy and by observation mechanism will provide means to correct these priors.

% What are the best 

% \section{Evolutionary dynamics of strategies}

% Mechanism of payoff

% payoff reads ...

% replicator dynamics ...

% % + rewrite abstract to be a bit better
% \clearpage



% \subsection*{Research questions}
% \begin{itemize}
%     \item Does learning by analogy based expectations converge towards Nash or ABE equilibrium in p-Beauty Contests (Keynes, 1936)\footnote{Possibly also/or centipede games} games with cognitive hierarchy of players? 
    
%     \item If yes, how does learning speed interplay with the levels of reasoning and the its distribution? The proportions of silly/sophisticated players?
    
%     \item Does being cognitively sophisticated grant higher payoffs in this context?\footnote{If I am very sophisticated in my guess, but alone to make that guess (many silly players), my guess will not be good. Overcoming this issue may require the agents to form expectations about the proportions of levels of reasoning in the population}
    
%     \item If learning by analogy based expectations with cognitive hierarchies of players converges to the Nash equilibrium, for large populations, can it explain and replicate experimental results of (Nagel, 1995; Duffy and Nagel, 1997, Ha, Camerer and Weiglet, 1998)
% \end{itemize}

% \textbf{Main intuition}: Beauty Contests Game are often finite and dominant solvable. In principle, both Nash and ABE Equilibria should exist. The Analogy-based approach would converge to the ABEE, and the Level K approach to the Nash. But what would be the result of a combination, to both account for learning and cognitive abilities of the players? Would it systematically converge to one of the two, or would it create multiple equilibria, depending on the distribution of levels of reasoning in the population? Additionally, to the best of my knowledge, the ABEE in the p-Beauty Contest Game hasn't been identified yet.

% \subsection*{Methods sketch}
% The idea is to mix both standard analytical methods to conduct a mathematical analysis in large populations, and an agent-based simulation with Monte Carlo methods to try to establish that these results are robust in situations with very small populations. The idea is to try to replicate the experimental results insights (Nagel, 1995; Duffy and Nagel, 1997, Ha, Camerer and Weiglet, 1998) both in large populations, and in replicating experimental conditions. The flexibility of computer modelling allows to replicate the material conditions of the experiment, and to test the theory (analogy K reasoning) over a very high number of draws: would an analogy-based K level theory of learning be relevant to explain the convergence to Nash equilibrium in these games with few rounds and few players? Or would it converge to something else? That way, comparing the results (convergence speed, learning paths), we may understand more precisely what the players need to learn in models to replicate empirical games trajectories.

% \textbf{Replication of experimental conditions and robustness of the results in finite populations}
% \begin{itemize}
%     \item In P-guessing games experimental settings, the agents only observe the average behavior, and their own payoffs.
%     \item Artificial experiments in a computer simulation, and the modelling of individual learning processes, can help establish the theoretical results (in large populations) in finite (experimental: 3 or 7 persons) groups of players.
% \end{itemize}

% \subsection*{Model outline}
% Adaptation of Analogy based reasoning (Jehiel, 1995); Huck, Jehiel \& Rutter, 2011) in the context of P-guessing games with the level K approach. Agents play to guess the p times average guess. Each game round fuels an analogy class, where the average behavior is recorded. Agents with learning abilities hence best respond to this expected average behavior.
% However, when they do so, cognitive abilities in the Level K approach enter into account. Sophisticated players anticipate that some players will best respond to the average behavior, and will best respond to these players.\footnote{Bundling of players and nodes may be crucial to get convergence to Nash, or convergence to something else (or pure divergence). If players bundle all players and all nodes together, convergence to Nash may be slow, or directed towards an ABEE.}\\

% \begin{itemize}
%     \item Level 0 : Random choice (no learning)
%     \item Level 1 : best response to observed average
%     \item Level 2 : best response to Level 1 action
% \end{itemize}

% As the experimental results, this model could be applied to both finite and infinite threshold games (Ho, Camerer and Weigelt, 1998), or variations of (Nagel, 1997) with median, maximum and mean games.\\
